IndicXNLI: Evaluating Multilingual Inference for Indian Languages

While Indic NLP has made rapid advances recently in terms of the availability of corpora and pre-trained models, benchmark datasets on standard NLU tasks are limited. To this end, we introduce IndicXNLI, an NLI dataset for 11 Indic languages. It has been created by high-quality machine translation of the original English XNLI dataset and our analysis attests to the quality of IndicXNLI. By finetuning different pre-trained LMs on this IndicXNLI, we analyze various cross-lingual transfer techniques with respect to the impact of the choice of language models, languages, multi-linguality, mix-language input, etc. These experiments provide us with useful insights into the behaviour of pre-trained models for a diverse set of languages.

==> automatic_scores_table.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with

%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htbp]
\centering
\small
% \scriptsize
\begin{tabular}{m{7em}<{\centering}|m{8em}<{\raggedright}|m{2em}<{\centering}|m{1.2em}m{1.2em}m{1.2em}m{1.2em}m{1.2em}m{1.2em}m{1.2em}m{1.2em}m{1.2em}m{1.2em}m{1.8em}<{\centering}}\toprule
\textbf{Strategy}& \textbf{Translation Model} & \textbf{Score} & \textbf{as} & \textbf{gu} & \textbf{kn} & \textbf{ml} & \textbf{mr} & \textbf{or} & \textbf{pa} & \textbf{ta} & \textbf{te} & \textbf{bn} & \textbf{hi} \\
\midrule
& & \textbf{F1} &0.93 &0.94 &0.94 &0.94 &0.93 &0.93 &0.94 &0.94 &0.94 &0.98 &0.98 \\
&\textbf{ IndicTrans} & \textbf{P} &0.92 &0.94 &0.93 &0.93 &0.93 &0.93 &0.94 &0.93 &0.93 &0.98 &0.98 \\
\textbf{Back Translated} & & \textbf{R} &0.93 &0.95 &0.94 &0.94 &0.94 &0.94 &0.95 &0.94 &0.94 &0.98 &0.98 \\
\cdashline{2-14}
& &\textbf{ F1 }&NA &0.94 &0.93 &0.92 &0.93 &0.91 &0.92 &0.92 &0.93 &0.94 &0.94 \\
& \textbf{Google Translate} &\textbf{ P} &NA &0.94 &0.93 &0.92 &0.92 &0.91 &0.92 &0.92 &0.93 &0.93 &0.94 \\
&& \textbf{R}&NA &0.94 &0.94 &0.92 &0.93 &0.91 &0.93 &0.93 &0.94 &0.94 &0.95 \\
\midrule
&&\textbf{F1} &0.85 &0.88 &0.87 &0.87 &0.86 &0.86 &0.88 &0.87 &0.87 &0.96 &0.96 \\
&\textbf{IndicTrans} & \textbf{P} &0.84 &0.87 &0.87 &0.86 &0.85 &0.85 &0.88 &0.86 &0.86 &0.96 &0.96 \\
 \textbf{Multilingual }&& \textbf{R} &0.86 &0.88 &0.88 &0.88 &0.87 &0.87 &0.89 &0.88 &0.88 &0.97 &0.96 \\
\cdashline{2-14}
 && \textbf{F1} & NA &0.89 &0.88 &0.85 &0.87 &0.82 &0.86 &0.86 &0.88 &0.89 &0.9 \\
&\textbf{Google Translate} &\textbf{P}&NA &0.88 &0.88 &0.84 &0.86 &0.82 &0.85 &0.85 &0.87 &0.88 &0.89 \\
&& \textbf{R} &NA &0.9 &0.89 &0.86 &0.88 &0.83 &0.87 &0.87 &0.89 &0.89 &0.9 \\
\bottomrule
\end{tabular}
\caption{Automatic Scores: Here Back Translated Strategy refers the the BERTScore between the original english and back translated sentence and Multilingual Strategy refers to BERTScore between english and indic sentences. P and R means precision and recall respectively}\label{tab: automatic scores}
\end{table*}

==> conclusion.tex <==
\section{Conclusion}
\label{ref:conclusion}

With \datasetName we extend the {\sc XNLI} dataset for \emph{Indic} languages family. We benchmark several multi-lingual models with various train-test strategies on \datasetName. We study the effects of using English {\sc XNLI} as pre-finetuning data. Furthermore, we also evaluate models on mixed-language inference input and cross-lingual transfer ability. We aim to integrate \datasetName and benchmark models in IndicGLUE \cite{kakwani-etal-2020-indicnlpsuite}. We also intend to enhance \datasetName with advanced translation techniques. Another direction is accessing model performance on {\sc Indic-IndicXNLI} task,  where both premises and hypothesis are in two distinct \emph{Indic} languages. 

==> experiments.tex <==
\section{Experiments Setup}
The objective of our experiments is to study how different multi-lingual models, including the one trained specifically for \emph{Indic} languages perform on the \datasetName dataset. We first discuss several multi-lingual models explored in our study.

\paragraph{Multi-lingual models.} For our experiments, we consider two categories of multi-lingual models, \begin{inparaenum}[(a)] \item \emph{Indic} specific: these models are specially pre-trained using Mask Language Modeling (MLM) or Translation Language Model (TLM) \citep{conneau2019cross} on monolingual / bilingual \emph{Indic} language corpora. These include models such as IndicBERT and MuRIL, and \item Generic: include massive multi-lingual models pre-trained large number of languages (typically around 100) with MLM such as XLM-RoBERTa and mBERT. 
% \vg{maybe we can describe models in the appendix and just put something brief here like Indic generic - mBERT, XLM-Roberta and Indic specific IndicBert and MuRIL because we have talked about them intro also, and this is quite self-explanatory.}
\end{inparaenum} \\

\noindent \textit{\emph{Indic} specific}: These include models such as MuRIL and IndicBERT trained on 17 and 11 \emph{Indic} languages ($+$English) respectively. MuRIL is pre-trained using Common-Crawl Oscar Corpus \cite{OrtizSuarezSagotRomary2019}, PMIndia \cite{haddow2020pmindia} on the following languages: \emph{en, hi, bn, ta, ur, ml, te, mr, new, kn, gu, pa, sd, or, as, say, ks}. IndicBERT is pre-trained using \emph{Indic}-Corp \cite{kakwani-etal-2020-indicnlpsuite} on the following languages: \emph{en, hi, bn, ta, ml, te, Mr, kn, gu, pa, or, as}. Moreover, MuRIL is also pre-trained with TLM objective (with MLM objective) on machine translated data and machine transliterated data.\\
% , such as Samantar, Common Crawl Oscar corpus \cite{ortiz-suarez-etal-2020-monolingual}, PMINDIA \cite{haddow2020pmindia} and  (\da{can you mention pre-train corpus here with citation Samantar and Indic corpus. check for the MuRIL work also, mention model also name and citation Ans: MuRIL is trained in Oscar Corpus and Wikipedia})

\noindent \textit{\emph{Generic}}: These include models such as multi-lingual BERT i.e. mBERT (cased/uncased) and multi-lingual RoBERTa i.e. XLM-RoBERTa which are train on a large number of languages.
XLM-RoBERTa also includes pre-training on all eleven \emph{Indic} languages. XLM-RoBERTa is pre-trained using the common crawl monolingual data. mBERT (cased/uncased) includes pre-training on nine of eleven \emph{Indic} languages (Assamese and Odia are not included in pre-training) and uses multi-lingual Wikipedia data for pre-training.

For all the discussed multi-lingual models, we build NLI classifiers by finetuning the pre-trained models. The classifier takes two sentence as input, i.e. the premise and the hypothesis as input and predicts the inference label. See Appendix \S\ref{sec:hyperparameters} for model hyper-parameters  details.

% For our experiments, we used  5 multi-lingual which can be divided into 2 categories, generalised multi-lingual models and Indic specific multi-lingual models. General multi-lingual models used were multi-lingual bert base cased, multi-lingual bert base uncased \cite{devlin2019bert} and xlm-roberta-base \emph{(XLM-R)} \cite{conneau2020unsupervised} while Indic specific models used were \emph{Indic}BERT (\emph{Indic}BERT) \cite{kakwani2020indicnlpsuite} and MuRIL-base-cased \cite{khanuja2021MuRIL}. The details of the hyper-parameters used for each model setting is given in \textbf{tab: \ref{tab: hyper-params}}

\paragraph{Training-Evaluation Strategies} 
To train the NLI classifier, we investigate several strategies. These strategies differ on the dataset we used for training and evaluation while keeping the underlying pre-trained multi-lingual models constant. Next, we describe these strategies in detail.

\begin{enumerate}[noitemsep]
    \item \textbf{\emph{Indic} Train} \label{strat:indic train}: The models are trained and evaluated on  \datasetName. This is the \textit{translate-train} scenario since the training set is translated from the original English dataset.
    
    \item \textbf{English Train} \label{strat:english train}: The models are trained on original English {\sc XNLI} data and evaluated on \datasetName data. This is a \textit{zero-shot evaluation} training scenario. 
    
    \item \textbf{English Eval}\label{strat:english eval}: The model are trained on original English {\sc XNLI}  data, but evaluated on English translation of \datasetName data. This is the \textit{translate-test} scenario.
    
    \item \textbf{English + \emph{Indic} Train} \label{english + indic train}: This approach combines approaches (1) and (2). The model is first pre-finetuned \citep{lee-etal-2021-meta,aghajanyan2021muppet} on English {\sc XNLI} data and then finetuned on \textbf{individual \emph{Indic} language} of \datasetName data.  
    
    \item \textbf{Train All} \label{train all}: This approach first pre-finetunes the pre-trained model on English {\sc XNLI} data followed by training on \textbf{all the eleven \emph{Indic} languages} jointly.
    
\end{enumerate}

% we need to do the random order experiments as 

For all strategies, the development set of \datasetName is similar, i.e. in the same language as the evaluation set of \datasetName. 

\subsection{\datasetName Results and Analysis}

In this section, we discuss the performance (accuracy) of multi-lingual models with varying training strategies for \datasetName inference task. We try to answer the following research questions:

\begin{enumerate}[noitemsep]
\item \textbf{RQ1:} How does models perform on \datasetName. Are \emph{Indic} languages pre-trained (i.e. \emph{Indic}-specific) model better? (\S\ref{sec:language_specific})
\item \textbf{RQ2:} Is it desirable to train and evaluate the models on the English translated \datasetName data? (\S\ref{sec:english_language_model})
\item \textbf{RQ3:} Can we enhance models performance on \datasetName using
English {\sc XNLI} as additional training data?  (\S\ref{sec:english_language_augmentation})
\item \textbf{RQ4:} Is the performance of the unified \emph{Indic} model better than the independent language specific \emph{Indic} models? (\S\ref{sec:unified_model})
\end{enumerate}

\subsubsection{\datasetName multi-lingual models. ({RQ1})}
\label{sec:language_specific}

This correspond to the \textbf{\emph{Indic} Train} setting, where model is train and evaluated on each \emph{Indic} languages independently. Table \ref{tab:RQ_1234} shows the multi-lingual models performance. \\

% \begin{table*}[ht]\centering
% \small
% \begin{tabular}{l|rrrrrrrrrrr|c}\toprule
% \textbf{Model} & \textbf{as} & \textbf{gu} & \textbf{kn} &\textbf{ml} & \textbf{mr}& \textbf{or} & \textbf{pa} & \textbf{ta} & \textbf{te} & \textbf{bn} & \textbf{hi} & \textbf{Model-Avg} \\\midrule
% \textbf{XLM-R} &\textcolor{BrickRed}{\textbf{70}} &73 &\textcolor{BrickRed}{\textbf{75}} &70 & \textcolor{BrickRed}{\textbf{75}} &32 &71 &76 &76 &\textcolor{BrickRed}{\textbf{76}} &\textcolor{ForestGreen}{\textbf{78}} &70 \\
% \textbf{IndicBert} &67 &69 &68 &60 &68 &69 & \textcolor{ForestGreen}{\textbf{73}} &37 &62 &70 &68 &65 \\
% \textbf{mBERT-cased} &71 &62 &69 &71 &71 &35 &70 &70 &69 &67 & \textcolor{blue}{\textbf{74}} &66 \\
% \textbf{MuRIL} &70 & \textcolor{ForestGreen}{\textbf{78}} & \textcolor{BrickRed}{\textbf{75}} &\textcolor{BrickRed}{\textbf{76}} &70 &\textcolor{BrickRed}{\textbf{76}} &72 & \textcolor{BrickRed}{\textbf{74}} & \textcolor{ForestGreen}{\textbf{78}} &75 &71 &\textbf{74} \\
% \textbf{mBERT-uncased} &64 &64 &63 &66 &65 &35 &68 &67 &67 &62 & \textcolor{blue}{\textbf{72}} &63 \\
% \hline
% \textbf{Lang-Avg} &68 &69 &70 &69 &70 &49 &71 &65 &70 &70 &\textbf{72} &68 \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{\emph{Indic} Train} model performance (refer \S \ref{sec:language_specific} {RQ1}). Here, Lang-Avg represents the language wise average score for all models while Model-Avg average score represents average score of a model across all languages. \da{what does green red and blue represent mention here} values in \textcolor{blue}{Blue} represents the model wise best score, while \textcolor{red}{Red} represents language wise average and \textcolor{ForestGreen}{Green} represents the values where model-wise average and language-wise average coincide.}
% \label{tab: translate-train}
% \end{table*}

% \begin{table*}[htb]\centering
% \small
% \begin{tabular}{l|rrrrrrrrrrr|c}\toprule
% \textbf{Model} & \textbf{as} & \textbf{gu} & \textbf{kn} &\textbf{ml} & \textbf{mr}& \textbf{or} & \textbf{pa} & \textbf{ta} & \textbf{te} & \textbf{bn} & \textbf{hi} & \textbf{Model-Avg} \\\midrule
% \textbf{XLM-R} &65 & \textcolor{red}{\textbf{66}} &69 &\textcolor{red}{\textbf{69}} &67 & \textcolor{red}{\textbf{67}} &61 &71 &69 &69 &\textcolor{blue}{\textbf{73}} & 69 \\
% \textbf{IndicBert} &57 &63 &53 &42 &59 &57 &\textcolor{blue}{\textbf{66}} &41 &56 &48 &63 &60 \\
% \textbf{mBERT-cased} &51 &57 &57 &57 &54 &34 &59 & \textcolor{blue}{\textbf{61}} &59 &57 &67 &59 \\
% \textbf{MuRIL} &\textcolor{red}{\textbf{68}} &32 & \textcolor{red}{\textbf{75}} &34 & \textcolor{red}{\textbf{68}} &\textcolor{red}{\textbf{67}} &\textcolor{red}{\textbf{70}} &\textcolor{red}{\textbf{74}} &\textcolor{red}{\textbf{71}} &\textcolor{red}{\textbf{74}} &\textcolor{ForestGreen}{\textbf{76}} &\textbf{72} \\
% \textbf{mBERT-uncased} &49 &55 & \textcolor{blue}{\textbf{64}} &59 &57 &35 &58 &60 &58 &62 &61 &55\\
% \hline
% \textbf{Lang-Avg} &58 &55 &64 &52 &61 &52 &63 &61 &63 &62 &\textbf{68} &63 \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{english train:} model performance (refer \S \ref{sec:english_language_model} {RQ2}). \textbf{Model-Avg} and \textbf{Lang-Avg} means the same as mentioned in \textbf{tab: \ref{tab: translate-train}}.}\label{tab: crosslingual-transfer}
% \end{table*}

% \begin{table*}[htb]\centering
% \small
% \begin{tabular}{l|rrrrrrrrrrr|c}\toprule
% \textbf{Model} & \textbf{as} & \textbf{gu} & \textbf{kn} &\textbf{ml} & \textbf{mr}& \textbf{or} & \textbf{pa} & \textbf{ta} & \textbf{te} & \textbf{bn} & \textbf{hi} & \textbf{Model-Avg} \\\midrule
% \textbf{XLM-RoBERTa}  & \textcolor{red}{\textbf{66}} & \textcolor{red}{\textbf{72}} & 70 & \textcolor{red}{\textbf{68}} & \textcolor{red}{\textbf{66}} & 65 & \textcolor{red}{\textbf{72}} & 69 & \textcolor{red}{\textbf{72}} & 71 &\textcolor{blue}{\textbf{75}}&\textbf{70} \\
% \textbf{\emph{Indic}BERT} & 63 & 66 & 68 & 61 & 65 & 65 & 66 & 63 & 63 &\textcolor{blue}{\textbf{72}} &\textcolor{blue}{\textbf{72}}& 66 \\
% \textbf{mBERT-cased} & 62 & 64 & 67 & 65 & 61 & 60 & 66 & \textcolor{red}{\textbf{67}} & 66 &\textcolor{blue}{\textbf{75}} & 72 & 66 \\
% \textbf{MuRIL} & 65 & 33 & \textcolor{red}{\textbf{71}} & 67 & 67 & \textcolor{red}{\textbf{67}} & 71 & 31 & 71 & 72 & \textcolor{ForestGreen}{\textbf{77}} & 63 \\
% \textbf{mBERT-uncased} & 61 & 65 & 61 & 65 & 56 & 66 & 69 & 70 & 67 &\textcolor{ForestGreen}{\textbf{76}}& 74 & 66 \\
% \hline
% \textbf{Lang-Avg} & 64 & 60 & 68 & 65 & 63 & 64 & 69 & 60 & 68 & 73 &\textbf{74}& 66 \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{english eval:} model performance (refer \S \ref{sec:english_language_model} {RQ2}). \textbf{Model-Avg} and \textbf{Lang-Avg} means the same as mentioned in \textbf{tab: \ref{tab: translate-train}}.}\label{tab: translate-test}
% \end{table*}

% \begin{table*}[htbp]\centering
% \small
% \begin{tabular}{l|rrrrrrrrrrr|c}\toprule
% \textbf{Model} & \textbf{as} & \textbf{gu} & \textbf{kn} &\textbf{ml} & \textbf{mr}& \textbf{or} & \textbf{pa} & \textbf{ta} & \textbf{te} & \textbf{bn} & \textbf{hi} & \textbf{Model-Avg} \\
% \midrule
% \textbf{XLM-RoBERTa}  & \textcolor{red}{\textbf{73}} & 75 & \textcolor{red}{\textbf{77}} & 75 & \textcolor{red}{\textbf{74}} & 73 & 75 & 75 & 73 & \textcolor{red}{\textbf{75}} & \textcolor{ForestGreen}{\textbf{79}} & 76 \\
% \textbf{\emph{Indic}BERT} & 67 & 72 & 65 & 62 & 59 & 59 &\textcolor{blue}{\textbf{74}} & 63 & 66 & 69 &\textcolor{blue}{\textbf{74}}&70 \\
% \textbf{mBERT-cased} & 67 & 70 & 69 & 70 & 70 & 39 & 71 &\textcolor{blue}{\textbf{73}} & 70 & 70 &71 & 69 \\
% \textbf{MuRIL} & 76 & \textcolor{red}{\textbf{77}} & 77 & \textcolor{ForestGreen}{\textbf{79}} & 74 & \textcolor{red}{\textbf{76}} &\textcolor{ForestGreen}{\textbf{77}} &\textcolor{ForestGreen}{\textbf{77}}& \textcolor{red}{\textbf{74}} & \textcolor{red}{\textbf{75}} &\textcolor{blue}{\textbf{77}}& \textbf{77} \\
% \textbf{mBERT-uncased} & 64 & 69 & 63 & 73 & 67 & 35 & 68 & 69 & 68 & 72 & \textcolor{blue}{\textbf{74}} & 69 \\
% \hline
% \textbf{Lang-Avg} & 69 & 73 & 70 & 72 & 68 & 56 & 73 & 72 & 70 & 72 &\textbf{75} & 72 \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{english + \emph{Indic} train:} model performance (refer \S \ref{sec:english_language_augmentation} {RQ3}). \textbf{Model-Avg} and \textbf{Lang-Avg} means the same as mentioned in \textbf{tab: \ref{tab: translate-train}}.}\label{tab: crosslingual transfer plus translate-train}
% \end{table*}

% \begin{table*}[htbp]\centering
% \small
% \begin{tabular}{l|rrrrrrrrrrr|c}\toprule
% \textbf{Model} & \textbf{as} & \textbf{gu} & \textbf{kn} &\textbf{ml} & \textbf{mr}& \textbf{or} & \textbf{pa} & \textbf{ta} & \textbf{te} & \textbf{bn} & \textbf{hi} & \textbf{Model Avg} \\\midrule
% \textbf{XLM-RoBERTa}  &\textcolor{red}{\textbf{73}} &\textcolor{ForestGreen}{\textbf{77}} &\textcolor{red}{\textbf{74}} &\textcolor{red}{\textbf{76}} &72 &73 &\textcolor{blue}{\textbf{77}} &\textcolor{blue}{\textbf{77}}&\textbf{76} &\textcolor{blue}{\textbf{77}}&\textcolor{blue}{\textbf{77}} &75 \\
% \textbf{\emph{Indic}BERT} & 63 & 74 & 59 & 51 & 69 & 66 &\textcolor{blue}{\textbf{75}} & 60 & 67 & 70 & 74 & 66 \\
% \textbf{mBERT-cased} & 63 & 69 & 69 & 71 & 70 & 33 & 71 & 69 & 70 &\textcolor{blue}{\textbf{74}} & 72 & 66 \\
% \textbf{MuRIL} & \textcolor{red}{\textbf{73}} & 76 & \textcolor{red}{\textbf{74}} & \textcolor{red}{\textbf{76}} & \textcolor{red}{\textbf{74}} & \textcolor{red}{\textbf{78}} &\textcolor{ForestGreen}{\textbf{81}} & \textcolor{red}{\textbf{78}} & \textcolor{red}{\textbf{76}} & \textcolor{red}{\textbf{80}} & \textcolor{red}{\textbf{78}} &\textbf{77} \\
% \textbf{mBERT-uncased} & 67 & 70 & 69 & 67 & 67 & 4 & 71 & 73 & 67 &\textcolor{blue}{\textbf{75}} & 72 & 67 \\
% \hline
% \textbf{Lang-Avg} & 68 & 73 & 69 & 68 & 71 & 58 & 75 & 71 & 71 &\textbf{75} & 74 & 70 \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{train all:} model performance (refer \S \ref{sec:unified_model} {RQ4}). \textbf{Model-Avg} and \textbf{Lang-Avg} means the same as mentioned in \textbf{tab: \ref{tab: translate-train}}.}\label{tab: translate-train all}
% \end{table*}

% \noindent \textit{Results Analysis}. We observe that MuRIL shows the best average performance; this can be attributed to two reasons, the model  \begin{inparaenum}[(a.)] \item is pre-trained on \emph{Indic} languages, \item and has more parameters, i.e. deeper architecture with bigger embedding size. \end{inparaenum} On average most models give their best NLI performance on \emph{Hindi} (hi) language set of \datasetName. Furthermore, \emph{Odia} (or) language set of \datasetName, seem most challenging. On \emph{Odia} (or) larger multi-lingual models such as mBERT (cased/uncased) struggles for good performance. The poor performance of mBERT on Odia can be attributed to its arcane script \citep{pires-etal-2019-multilingual}. The poor performance can be attributed to the fact at mBERT, which can be attributed to the nature of script of \emph{Odia}. XLM-RoBERTa is at par with MuRIL despite being a generic model. The performance gains are maximum for the \emph{Hindi} (hi) language. This is because, among all these languages, \emph{Hindi} (hi) had the highest proportion of pre-training data on models, resulting in better improvements for the NLI models when trained on \emph{Hindi}. IndicBERT, despite being a smaller model, performs as good as mBERT (cased/uncased). This can be attributed to the \emph{Indic}-specific nature of the IndicBERT model.

% Additionally, on \emph{Indic} languages such as \emph{Odia}, \emph{`Malayali'} and \emph{`Gujarati'}, model train on language-specific data e.g. IndicBERT perform supervisor than XLM-RoBERTa and mBERT, despite smaller model parameters.

% This can be because it is trained on \emph{Indic} languages in its pre-training objective and is also one of the most significant models. 

% We also observe that Hindi has the largest language-wise average as it is the highest resource language we are considering. 

% Odia seems to be the most challenging language to handle for models like XLM-RoBERTaand mBERT, which emphasizes the significance of language-specific models for the NLP community. mBERT cased and XLM-RoBERTahas are the lowest-performing models, whereas \emph{Indic}BERT, which is a smaller model, performs better in some challenging languages like Odia, Malayali and Gujurati, which is also a considerably smaller model. 


\subsubsection{How well English {\sc XNLI} train model perform on \datasetName? ({RQ2})}
\label{sec:english_language_model}
Next, we discuss how we can leverage original  English {\sc XNLI} data for model training. We choose English because it is the most prominent language set on which  models are
\begin{inparaenum}[(a.)] \item  pre-trained using MLM or TLM objective with English corpus, \item  trained for Multi-Task objective for multiple tasks with English benchmark dataset, \item better at cross-lingual transferability with English training \cite{hu2020xtreme} \end{inparaenum}. 

\paragraph{English Train:} To test this, we experiment with \textbf{English Train} model which is train on the original English {\sc XNLI} data, and evaluated for \emph{cross lingual transfer} performance on the \emph{Indic} languages in \datasetName set. Training over high-resource English language benefit model for effective NLI task-adaptation. Table \ref{tab:RQ_1234} shows the  models performance. \\


% we want to see if training in English can help improve the accuracy of our models with different training combinations. 

% \subsubsection{Cross-lingual transfer: Can we use English data for training and test on Indic Languages?}
% In these experiments, we trained our models on original English language and tested them on Indic languages. The test and validation datasets were those obtained through translation.
% \\

% \noindent \textit{Results Analysis.}  On average, for all models, the cross-lingual transfer performance is best for \emph{Bengali} (bn) and \emph{Hindi} (hi) language. One possible explanation for this high-performance level is because multi-lingual models are pre-trained on quite large monolingual corpora of these two languages. Here too, MuRIL model performs best across most languages, while cross-lingual transfer on \emph{Hindi} (hi) is best for most models. 

% When, exclusively using English {\sc XNLI} data for training, the model's overall performance is worse than \emph{Indic}-specific language is used for training (i.e. \textbf{\emph{Indic} Train}), refer \S \ref{sec:language_specific} Table \ref{tab:RQ_1234}. We suspect this poor performance is because model fail to understand language-specific features. This proves the requirement of our \emph{Indic} languages specific \datasetName data for effective model training. However, the drop in performance was not drastic in comparison with the \textbf{\emph{Indic} Train} setting indicating that cross-lingual transfer after fine-tuning on English {\sc XNLI} data is a strong baseline.

% Despite lesser parameters, e.g. IndicBERT outperforms mBERT (cased/uncased), MuRIL out-performs XLM-RoBERTa. As earlier, in comparison to \emph{Indic} pre-train models such as MuRIL and IndicBERT, both XLM-RoBERTa and mBERT (cased/uncased) perform particularly poorly with \emph{Odia} (or) language. From this, we can infer that \emph{Indic}-specific pre-training is beneficial for the cross-lingual transfer task.

% However, when exclusively using English data for training, the model's overall performance is worse than when all \emph{Indic}-specific language is used for training ( i.e. \textbf{\emph{Indic} Train}), refer \S \ref{sec:language_specific} Table \ref{tab:RQ_1234}. 

% These are also the languages that are there in the pre-training objective of all models.

\paragraph{English Eval}: We further enhance \textbf{English Train} cross-lingual transferability, using English translated \datasetName evaluation set. To obtain an evaluation set in the English language, we use the IndicTrans translation model. The model performs \emph{Indic} to English translation of the \datasetName evaluating sets. This method of \emph{evaluation translation} effectively bridges the linguistic gap due to language variance between the training and the evaluation set. Table \ref{tab:RQ_1234} shows the multi-lingual model performance.  \\

% \subsubsection{Translate Test}
% In these set of experiments, every model was trained on original English data and was tested on back-translated English data from each Indic language. The data was back-translated from the translations obtained from Indic trans. Indic-trans was used for back-translation as well.
% \\
\input{tables_parta}

% \noindent \textit{Results Analysis:}  We observe that the performance of the multi-lingual model improves when tested on translated English data. This improvement is attributed to the model being trained and assessed on homogeneous resource-rich English language data. Furthermore, the models perform much better on \emph{Odia} (or) language when compared with previous strategies. Despite, substantial gain on \emph{Odia} (or), models still performs best for resource-rich \emph{Hindi} (hi) and \emph{Bengali} (bn) languages. The two reasons for this performance variation across languages are \begin{inparaenum}[(a.)] \item weaker \emph{Indic}-English translation by IndicTrans for low-resource \emph{Indic} languages, \item and, better pre-training (due to larger share in pre-training data) for \emph{Hindi} (hi) and \emph{Bengali} (bn) languages.
% \end{inparaenum} 

% XLM-RoBERTa appears to be the best model, which is unexpected given MuRIL's is \emph{Indic}-specific and of similar size (similar number of parameters). This shows that generic models perform better in English evaluation settings as compared to \emph{Indic}-specific models. The fact that the assessment and pre-training language are both English benefits these generic models.

% However, We can observe that the best performing languages are Hindi and Bengali, which are relatively high resources and are also part of the pre-training objective data of all models. 

\subsubsection{Does Pre-finetuning on English {\sc XNLI} help multi-lingual models? ({RQ3})}
\label{sec:english_language_augmentation}

% \subsubsection{Using English {\sc XNLI} as augmented training data. ({RQ3})}

% \subsubsection{Can training on English {\sc XNLI} help multi-lingual models?}

Several studies has shown that \emph{Pre-finetuning} approach \citep{lee-etal-2021-meta,aghajanyan2021muppet} i.e. early training a pre-trained model on similar task using augmented data benefits low-resource generalization through effective task-adaptation. We also use the English {\sc XNLI} data as augmented training data for \emph{``initial fine-tuning"} of model. We use the \textbf{English + \emph{Indic} Train} model, which is first trained on English {\sc XNLI} data followed by training on \textbf{individual \emph{Indic} language} of \datasetName. We use the same \emph{Indic} language for both training and evaluation for \textbf{English + \emph{Indic} Train} model.

% The language for each of the \emph{Indic} train data is the same as the language in which the model is evaluated.

Firstly, training on high resource English {\sc XNLI} data ensure models better adapt for the NLI task. Followed by training on the \textit{Indic} dataset, support the models in acquiring language specific aspects and cross-lingual transfer ability \citep{xu-etal-2021-gradual,gururangan-etal-2020-dont,aghajanyan2021muppet}. Thus we effectively combine the \textbf{English Train} model (for task adaptation) and \textbf{\emph{Indic} Train} model (for cross lingual and language-specific learning) in the \textbf{English + \emph{Indic} Train} model setting. Table \ref{tab:RQ_1234} shows the multi-lingual models performance.\\

% Training on English initially makes the model more robust because English is the dominant language in terms of pre-training data size. Hence, training in English first impacts the overall weights of the model during fine-tuning, and the model can get a general sense of the task itself. While training on the \emph{Indic} language later improves the model in the language-specific aspect. 

% In this set of experiments, we mixed the approach of cross-lingual transfer and translated train by training the models twice.  The model was then tested on the test set of the translated Indic language data.

% English training improves the model consistency for many models, i.e. the model performs reasonably well for all the languages. This can be due to the phenomenon that English helps in `meta-learning for the model and then \emph{Indic}-training helps in language-specific learning.

% \noindent \textit{Results Analysis:}
% Overall, we observe that English followed by \emph{Indic} language training tends to enhance the performance for all models. As earlier, MuRIL gives the best performance average for most languages, and \emph{Hindi} has the best performance on average across all models. The technique has the best overall accuracy of 72 i.e. aggregated average overall models and languages. The sole downside of this technique is that it has double training time due to both English and \emph{Indic} language training. Moreover, mBERT (uncased/cased) still perform poorly on \emph{Odia} (or) language.
% \\
% % \vspace{-0.3cm}
% Again, we observe an evident performance benefit to \emph{Indic}-specific models, because of similar reasons as described in the previous section \S \ref{sec:language_specific}. Moreover, \emph{Indic}-specific models reap benefits of having evaluation data in \emph{Indic} language. We also observe the reduced variance in performance across languages for all models. Despite this, the performance for high resource \emph{Hindi} (hi) and \emph{Bengali} (bn) languages remains the best.\\
% English training also takes longer to converge than other languages, resulting in a strong foundation for the model about the task that can be fine-tuned using language-specific data.
\subsubsection{Unified \datasetName multi-lingual inference model. ({RQ4})}
\label{sec:unified_model}
Until recently, we had been creating independent inference models for each \emph{Indic} language through various settings. However, prior work on translation has demonstrated that multi-lingual models trained together on multiple closely related languages always perform better than individual bilingual models \cite{ramesh2021samanantar}. On similar lines, we increase the languages exposure for NLI models by training the model on \textbf{all the eleven \emph{Indic} languages together} i.e. \textbf{Train All} setting. In \textbf{Train-all} we create a unified multi-lingual model by first training on English {\sc XNLI} followed by training the same model on \textbf{all the eleven \emph{Indic} languages} i.e. complete \emph{Indic} language family of \datasetName.  

This \textbf{Train All} techniques has multiple benefits, as follows \begin{inparaenum}[(a.)] \item single unified model work across all \emph{Indic} languages, instead of language-specific several individuals models. \item Overall training time is also drastically reduced, compare to \textbf{English + \textit{Indic} Train} model the \textbf{Train All} model is $2\times$ faster to train. \item since the same model has trained for all \emph{Indic} languages at once, and the model performs consistently across all languages. For individual models, the amount of pre-training data available in each language can substantially impact their performance. \item and model exploit inter-language similarities for better cross-lingual transfer capacity. \end{inparaenum} Table \ref{tab:RQ_1234} show performance of multi-lingual models. \\

% In this set of experiments, we are trying to increase the language exposure of our models.  We obtained significant performance gains and also obtained a single unified model for all languages. 

% \noindent \textit{Results Analysis.} Overall we observe that single unified model \textbf{Train All} perform much better than individual models i.e. \textbf{English + \emph{Indic} Train}, refer to \S\ref{sec:unified_model}. This lends credence to the argument that unified models developed for closely related languages outperform individual models developed for each language \citep{tan2019multilingual}. The \textbf{Train All} method may alternatively be viewed as an extension of English {\sc XNLI} augmentation, now with remaining \datasetName \emph{Indic} languages as additional augmentation data. MuRIL performs best for all languages across models on average. As earlier \emph{Hindi} and \emph{Bengali} has better performance as compared to other \emph{`Indic'} languages.

% Like earlier sections that models tend to favour high resource languages like \emph{Hindi} and \emph{Bengali} and sometimes can show higher gains for these languages. This problem is more or less improved with this approach, as we can now see that for each model, the accuracy is evenly distributed for every language. 


\subsection{\datasetName Cross-Lingual Transfer}
\label{sec:indic_crosslingual}

In this section, we try to answer the following research question. 

\paragraph{RQ5:} Can language specific model (\S\ref{sec:language_specific}) transfer performance across \emph{Indic} languages? \\

\input{tables_partb}

\noindent In response to RQ5, we evaluate language specific model (\S\ref{sec:language_specific}) on their Cross-lingual transfer ability across \emph{Indic} languages i.e. evaluating performance of model train on "X" \emph{Indic} language on "Y" \emph{Indic} language. We trained the model with the \textbf{\emph{Indic}} Train setting. However, we evaluated each \emph{Indic} language model performance across all \textbf{\emph{Indic}} languages. Table \ref{tab:indic_crosslingual_summary} present the average evaluation score of all \emph{Indic} language when train on the mentioned column language of \datasetName. For detailed model-wise cross-lingual train-test language results, refer to Appendix 
\S\ref{sec:indic_crosslingual_appendix}. \\

% \noindent \textit{Results Analysis:} As earlier, we observe that the models tend to favour high resource languages \emph{Hindi} and \emph{Bengali} training for better cross-lingual transfer. Because of the higher amount of monolingual corpus, more frequent pre-training for these languages may be one explanation for improved performance \cite{conneau2020unsupervised}. One can think of this as replacing English training \S \ref{sec:english_language_model} with \emph{Hindi} and \emph{Bengali} training. Furthermore, model train on non-\emph{Hindi} and non-\emph{Bengali} when evaluated for all \emph{Indic} languages perform best for the \emph{Hindi} and \emph{Bengali} language.
% Except for MuRIL and IndicBERT, which gain from \emph{Indic}-specific pre-training, \emph{Odia} is a difficult language for all other models. MuRIL performs the best amongst all models. We observe a strong correlation between \emph{Indic}-specific pre-training and model performance. We also observe that larger model size and \emph{Indic}-specificity benefit model performance. 

From detailed results in Appendix \S\ref{sec:indic_crosslingual_appendix}, we observe that models have relatively low diagonal correlation, i.e. models may not necessarily perform best on evaluation on the training language. This also demonstrates that selecting the appropriate language for cross-lingual transfer can significantly boost the odds of obtaining a better overall model. 

% We observe that model performance is biased towards \emph{Hindi} and \emph{Bengali} languages. 

% Moreover, fine-tuning on \emph{Hindi} benefits most in cross-lingual transfer performance. 

% We observe that \emph{Hindi} cross-lingual transfer can give strong baselines. 

% We also observe that independent of training language models transfer best for \emph{Hindi} and \emph{Bengali} languages.



% with the benefits of Indic specific pre-training in this section with the model performance. 

% For \textbf{XLM-RoBERTa}, the model perform best for the \textit{`Bengali'} language. The model gives the best performance average across all other languages if trained on \textit{`Bengali'}. A model trained in other languages, on average, also performs best for \textit{`Bengali'} language. XLM-RoBERTa also struggles to correlate with \textit{`Kannada}, \textit{`Odia}, and \textit{`Malayalam}, thus performs poorly on average if trained for them. At the same time, all models have poor cross-lingual ability transferability for the \textit{`Assamese'} language. Furthermore, XLM-RoBERTa seems to perform better when trained and evaluated for higher resource languages such as \textit{`Bengali'} and \textit{`Hindi'}. 

% For \textbf{IndicBERT}, the overall score is comparable to XLM-RoBERTa despite it being a significantly smaller model. On average, across languages, the cross-lingual transferability for models trained on varying \emph{Indic} languages were consistently similar (between 0.5 - 0.6). However, the evaluation performance for cross-lingual models evaluated on \emph{`Malayalam'} was poor for all \emph{Indic} trained models. For model trained on some languages, \emph{`Kannada'}, \emph{`Malayalam'} and \emph{`Punjabi'}, the best performance was across diagonal, i.e. indicating the model performs best on the trained language. This trend was, however, surprisingly not valid in other \emph{Indic} languages, indicating remarkable cross-lingual transferability of \emph{Indic}BERT model.

% For \textbf{mBERT-cased}, the model performs worse for \textbf{`Odia'} on avergae for both when evaluated and train on. However, all models performs very consistently for other \textit{Indic} languages. Model trained on \textit{Kannada}, \textit{Punjabi}, \textit{Tamil}, \textit{Hindi}, and \textit{Bengali} perform best on average across languages. Here too, the best cross-lingual transfer ability was shown for \textit{Bengali} language. mBERT-cased also for some languages have best performance across diagonal, i.e. the model performs the best on the language it is trained on, these languages include \textit{Assamese}, \textit{Gujurati}, \textit{Malayalam}, \textit{Punjabi} and \textit{Telugu}. 

% % \begin{table*}\centering
% % \small
% % \begin{tabular}{llrrrrrrrrrrrc}\toprule
% % \bf{Strategy} & \textbf{Model} & \textbf{as} & \textbf{gu} & \textbf{kn} &\textbf{ml} & \textbf{mr}& \textbf{or} & \textbf{pa} & \textbf{ta} & \textbf{te} & \textbf{bn} & \textbf{hi} & \textbf{Model Avg} \\\midrule
% % & \textbf{XLM-RoBERTa}  & 66 & 70 & 33 & 34 & 70 & 35 & 68 & 70 & 70 & 71 & \textcolor{blue}{\textbf{72}} & 60 \\
% % & \textbf{IndicBERT} & 59 & \textcolor{blue}{\textbf{60}} & 59 & 54 & \textcolor{blue}{\textbf{60}} & \textcolor{blue}{\textbf{60}} & \textcolor{blue}{\textbf{60}} & 56 & 59 & 58 & \textcolor{blue}{\textbf{60}} & 59 \\
% % \textbf{\emph{Indic} Train} & \textbf{mBERT uncased} & 59 & 59 & 60 & 59 & 58 & 33 & 59 & 60 & 60 & 59 & \textcolor{blue}{\textbf{61}} & 57 \\
% % & \textbf{MuRIL} & \textcolor{red}{\textbf{75}} & \textcolor{red}{\textbf{73}} & \textcolor{red}{\textbf{75}} &\textcolor{ForestGreen}{\textbf{76}}& \textcolor{red}{\textbf{71}} & 33 & \textcolor{red}{\textbf{75}} & \textcolor{ForestGreen}{\textbf{76}} & \textcolor{red}{\textbf{73}} & \textcolor{red}{\textbf{75}} & \textcolor{red}{\textbf{73}} & \textbf{70} \\
% % & \textbf{mBERT cased} & 57 & 59 & \textcolor{blue}{\textbf{60}} & 59 & 58 & 33 & 59 &\textcolor{blue}{\textbf{60}} & 59 & \textcolor{blue}{\textbf{60}} & \textcolor{blue}{\textbf{60}} & 57 \\
% % \hdashline
% % & \textbf{Lang-Avg} & 63 & 64 & 57 & 56 & 63 & 39 & 64 & 64 & 64 &\textbf{65} &\textbf{65} & 60 \\
% % \bottomrule
% % \end{tabular}
% % \caption{Summary of \textbf{\emph{Indic} Cross-lingual Transfer.} model (refer \S \ref{sec:indic_crosslingual} {RQ5}). Every row represents the train average of each languages if trained on that language and tested on all language. Model average means the same as mentioned in \textbf{tab:} \ref{tab: translate-train}. For detail results on \emph{Indic} Cross-lingual Transfer refer to Appendix \S\ref{sec:indic_crosslingual_appendix}. Here, \textbf{Model-Avg}, \textbf{Lang-Avg}, and color code represent the same as mentioned in \textbf{tab: \ref{tab:RQ_1234}} }\label{tab:indic_crosslingual_summary}
% % \end{table*}

% % \input{tables_partb}

% For \textbf{mBERT-uncased}, the model correlate poorly for \emph{Odia} language, however, shows similar results as mBERT-cased for all other languages. Model trained on \textit{Kannada} and \textit{Bengali} perform best on average across languages. Here too, the best cross-lingual transfer ability was shown for \textit{Bengali} language. mBERT-uncased also for some languages have best performance across diagonal, i.e. the model performs the best on the language it is trained on, these languages include \textit{Assamese}, \textit{Gujurati}, \textit{Malayalam}, \textit{Kannada} and \textit{Marathi}.

% \textbf{MuRIL} has the best overall cross-lingual transferability amongst all the models. \textbf{MuRIL} only fails to generalize well when trained for \textit{`Odia'} language. However, model train on other \emph{Indic} language when evaluated on \textit{`Odia'} performs well. Model trained on \textit{Marathi} and \textit{Marathi} perform best on average across languages. The best cross-lingual transferability was shown for \textit{Bengali} and \textit{Hindi} language. Muril shows diagonal correlation in performance with languages such as \textit{Marathi}, \textit{Odia} and \textit{Telugu}. Overall, MuRIL has better cross-lingual transferability across all languages compared to other models. It also reflects less performance bias for languages such as \textit{Bengali} and \textit{Hindi}, as compared to XLM-RoBERTa.



\subsection{{\sc{En-IndicXNLI}} Results and Analysis}
\label{sec:english-Indic}

\input{tables_partc}

In this section, we try to answer the following research question. We refer to {\sc{En-IndicXNLI}} as NLI task where the premise is in English and Hypothesis is in \emph{Indic} language. 

% \vg{you mentioned something about news coming in one language and asking some questions in another language in one of our discussions, maybe we can add that here to motivate this task better.}

% \begin{table*}[!htbp]\centering
% \small
% \begin{tabular}{l|rrrrrrrrrrr|c}\toprule
% \textbf{Model} & \textbf{as} & \textbf{gu} & \textbf{kn} &\textbf{ml} & \textbf{mr}& \textbf{or} & \textbf{pa} & \textbf{ta} & \textbf{te} & \textbf{bn} & \textbf{hi} & \textbf{Model Avg} \\\midrule
% \textbf{XLM-RoBERTa}  & \textcolor{red}{\textbf{74}} & \textcolor{red}{\textbf{72}} & \textcolor{red}{\textbf{75}} & \textcolor{red}{\textbf{74}} & \textcolor{ForestGreen}{\textbf{77}} & \textcolor{red}{\textbf{72}} & 70 & \textcolor{red}{\textbf{72}} & \textcolor{red}{\textbf{72}} & \textcolor{ForestGreen}{\textbf{79}} & \textcolor{red}{\textbf{76}} &\textbf{74} \\
% \textbf{\emph{Indic}Bert} & 70 & 68 & 63 & 65 & 69 & 68 &\textcolor{blue}{\textbf{71}} & 64 & 64 & 69 & 69 & 67 \\
% \textbf{mBERT-cased} & 51 & 56 & 59 & 50 & 62 & 31 & \textcolor{blue}{\textbf{63}} & 57 & 60 & 61 &\textcolor{blue}{\textbf{63}} & 56 \\
% \textbf{MuRIL} & 71 & 70 &\textcolor{blue}{\textbf{73}} & 69 & 71 & 39 & 71 & 71 & 69 & 72 & 69 & 67 \\
% \textbf{mBERT-uncased} & 60 & 57 & 61 & 61 & 59 & 56 & 36 & 59 & 69 &\textcolor{blue}{\textbf{74}}& 71 & 60 \\
% \hline
% \textbf{Lang-Avg} & 65 & 65 & 66 & 64 & 68 & 53 & 62 & 65 & 67 &\textbf{71} & 70 & 65 \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{english-\EMPH{Indic} {\sc XNLI} with english + \emph{Indic} training setting:} model performance (refer \S \ref{sec:english-Indic} {RQ6}). \textbf{Model-Avg} and \textbf{Lang-Avg} means the same as mentioned in \textbf{tab: \ref{tab: translate-train}}.}\label{tab: Indic-English Cross lingual Transfer plus Translate Train}
% \end{table*}

% \begin{table*}[!htbp]\centering
% \small
% \begin{tabular}{l|rrrrrrrrrrr|c}\toprule
% \textbf{Model} & \textbf{as} & \textbf{gu} & \textbf{kn} &\textbf{ml} & \textbf{mr}& \textbf{or} & \textbf{pa} & \textbf{ta} & \textbf{te} & \textbf{bn} & \textbf{hi} & \textbf{Model Avg} \\\midrule
% \textbf{XLM-RoBERTa}  & \textcolor{red}{\textbf{57}} & \textcolor{red}{\textbf{59}} & \textcolor{red}{\textbf{58}} & \textcolor{red}{\textbf{62}} & \textcolor{red}{\textbf{61}} & 53 & 57 & 59 & 
% \textcolor{red}{\textbf{61}} &\textcolor{ForestGreen}{\textbf{63}} &\textcolor{ForestGreen}{\textbf{63}} &\textbf{59} \\
% \textbf{\emph{Indic}BERT} & 49 & 53 & 46 & 37 & 52 & 51 & 59 & 39 & 51 &\textcolor{blue}{\textbf{57}} & 50 & 50 \\
% \textbf{mBERT-cased} & 39 & 39 & 43 & 38 & \textcolor{blue}{\textbf{43}} & 33 & 40 & 42 & 41 & 40 & 42 & 40 \\
% \textbf{MuRIL} & 51 & 52 & 58 & 56 & 53 & \textcolor{red}{\textbf{55}} & \textcolor{red}{\textbf{58}} &\textcolor{blue}{\textbf{65}} & 55 & 62 & 54 & 56 \\
% \textbf{mBERT-uncased} &40 & 42 & 49 & 46 & 48 & 34 & 46 & 45 & 45 &\textcolor{blue}{\textbf{48}} & 44 & 44 \\
% \hline
% \textbf{Lang-Avg} & 47 & 49 & 51 & 48 & 51 & 45 & 52 & 50 & 51 &\textbf{54} & 51 &50 \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{english-\EMPH{Indic} {\sc XNLI} with train all setting:} model performance (refer \S \ref{sec:english-Indic} {RQ6}). \textbf{Model-Avg} and \textbf{Lang-Avg} means the same as mentioned in \textbf{table: \ref{tab: translate-train}}.}\label{tab: English-Indic Translate Train All}
% \end{table*}

% \input{tables_partc}

\paragraph{RQ6:} How does \datasetName models (\S\ref{sec:english_language_augmentation} and \S\ref{sec:unified_model}) perform on {\sc{En-IndicXNLI}}?\\

\noindent In response to RQ6, we analysed the performance of multi-lingual models when premise is in English and hypothesis is in \textit{Indic} language. This task assesses the model's ability to perform abreast  (English-\emph{Indic}) \textbf{intra-input} cross-lingual reasoning. Therefore, we create {\sc{En-IndicXNLI}} dataset which contain English \emph{premises} from {\sc XNLI} and corresponding \emph{Indic} hypothesis from \datasetName. To asses this task, we train model on {\sc{En-IndicXNLI}} train set using \textbf{English + \emph{Indic} Train} ( \S\ref{sec:english_language_augmentation}) and \textbf{Train All} (\S\ref{sec:unified_model}) strategies except with English premises. During inference we evaluate on similar setting i.e. {\sc{En-IndicXNLI}} evaluation set. Table \ref{tab:RQ_6} shows performance of \textbf{English + \emph{Indic} Train} and \textbf{Train All} models on {\sc{En-IndicXNLI}}. \\

% \noindent \textit{Results Analysis.} We observed a performance loss except for XLM-RoBERTa when the model is evaluated on {\sc{En-IndicXNLI}} inference task. The inference models struggle to correlate and reason together on two different languages (English, \emph{Indic}) sentences. Contrary to earlier observation, a generic model such as XLM-RoBERTa outperforms the \emph{Indic} specific models. However, IndicBERT and MuRIL perform better than mBERT. \emph{Bengali} perform best for both the training strategies. We also observe the benefit of English data augmentation \textbf{English + \emph{Indic} Train} model, rather than all language augmentation \textbf{Train All} model. 
% This is due to the fact that the \textbf{English + \emph{Indic} Train} model does not train on \emph{Indic} languages that are not present in example, i.e. no cross-lingual transfer.

% We observe that \textbf{English + \emph{Indic} Train} perform better than  technique. 

% \noindent \textit{Overall Summary:} Overall we observe that model performance drops drastically on english-\emph{Indic} task. 

% This is particularly interesting because the English-Indic model adapts well to a variety of tasks and not just traditional \textit{NLI} tasks with sentences in the same languages. 

% This can be attributed to the fact that since our premise is in English when we initially fine-tune, the model "meta-learns" the task well and training on English-Indic data further fine-tunes the model with language-specific capabilities. 
% Train all fine-tuning setting tends to work a bit worse. This can be attributed to the fact that the internal model representation of the sentences degrades the internal representation due to the complexity of the task as we fine-tune our models gradually.






==> table_parta.tex <==
\begin{table*}[!ht]
\centering
\footnotesize
\begin{tabular}{llrrrrrrrrrrrc}\toprule
\textbf{Strategy} & \textbf{Model} & \textbf{as} & \textbf{gu} & \textbf{kn} &\textbf{ml} & \textbf{mr}& \textbf{or} & \textbf{pa} & \textbf{ta} & \textbf{te} & \textbf{bn} & \textbf{hi} & \textbf{ModelAvg} \\\midrule
& \textbf{XLM-RoBERTa} &\textcolor{BrickRed}{\textbf{70}} &73 &\textcolor{BrickRed}{\textbf{75}} &70 & \textcolor{BrickRed}{\textbf{75}} &32 &71 &76 &76 &\textcolor{BrickRed}{\textbf{76}} &\textcolor{ForestGreen}{\textbf{78}} &70 \\
& \textbf{IndicBERT} &67 &69 &68 &60 &68 &69 & \textcolor{ForestGreen}{\textbf{73}} &37 &62 &70 &68 &65 \\
\textbf{\emph{Indic} Train} & \textbf{mBERT-cased} &71 &62 &69 &71 &71 &35 &70 &70 &69 &67 & \textcolor{blue}{\textbf{74}} &66 \\
% \S \ref{sec:language_specific} {RQ1}
& \textbf{MuRIL} &70 & \textcolor{ForestGreen}{\textbf{78}} & \textcolor{BrickRed}{\textbf{75}} &\textcolor{BrickRed}{\textbf{76}} &70 &\textcolor{BrickRed}{\textbf{76}} &72 & \textcolor{BrickRed}{\textbf{74}} & \textcolor{Forest Green}{\textbf{78}} &75 &71 &\textbf{74} \\
% & \textbf{mBERT-uncased} &64 &64 &63 &66 &65 &35 &68 &67 &67 &62 & \textcolor{blue}{\textbf{72}} &63 \\
\hdashline
& \textbf{LanguageAvg} &68 &69 &70 &69 &70 &49 &71 &65 &70 &70 &\textbf{72} &68 \\
\midrule
% \end{tabular}
% \caption{\textbf{\emph{Indic} Train} model performance (refer \S \ref{sec:language_specific} {RQ1}). Here, Language-Avg represents the language wise average score for all models while Model-Avg average score represents average score of a model across all languages. \da{what does green red and blue represent mention here}}
% \label{tab: translate-Train}
% \end{table*}

% \begin{table*}[htb]\centering
% \small
% \begin{tabular}{l|rrrrrrrrrrr|c}\toprule
% \textbf{Model} & \textbf{as} & \textbf{gu} & \textbf{kn} &\textbf{ml} & \textbf{mr}& \textbf{or} & \textbf{pa} & \textbf{ta} & \textbf{te} & \textb  f{bn} & \textbf{hi} & \textbf{Model-Avg} \\\midrule
& \textbf{XLM-RoBERTa} &65 & \textcolor{BrickRed}{\textbf{66}} &69 &\textcolor{BrickRed}{\textbf{69}} &67 & \textcolor{BrickRed}{\textbf{67}} &61 &71 &69 &69 &\textcolor{blue}{\textbf{73}} & 69 \\
& \textbf{IndicBERT} &57 &63 &53 &42 &59 &57 &\textcolor{blue}{\textbf{66}} &41 &56 &48 &63 &60 \\
\textbf{English Train} & \textbf{mBERT-cased} &51 &57 &57 &57 &54 &34 &59 & \textcolor{blue}{\textbf{61}} &59 &57 &67 &59 \\
% \S \ref{sec:english_language_model} {RQ2} 
&\textbf{MuRIL} &\textcolor{BrickRed}{\textbf{68}} &32 & \textcolor{BrickRed}{\textbf{75}} &34 & \textcolor{BrickRed}{\textbf{68}} &\textcolor{BrickRed}{\textbf{67}} &\textcolor{BrickRed}{\textbf{70}} &\textcolor{BrickRed}{\textbf{74}} &\textcolor{BrickRed}{\textbf{71}} &\textcolor{BrickRed}{\textbf{74}} &\textcolor{ForestGreen}{\textbf{76}} &\textbf{72} \\
% & \textbf{mBERT-uncased} &49 &55 & \textcolor{blue}{\textbf{64}} &59 &57 &35 &58 &60 &58 &62 &61 &55\\
\hdashline
& \textbf{LanguageAvg} &58 &55 &64 &52 &61 &52 &63 &61 &63 &62 &\textbf{68} &63 \\
\midrule
% \end{tabular}
% \caption{\textbf{English Train:} model performance (refer \S \ref{sec:english_language_model} {RQ2}). \textbf{Model-Avg} and \textbf{LanguageAvg} means the same as mentioned in \textbf{table: \ref{tab: translate-Train}}.}\label{tab: crosslingual-transfer}
% \end{table*}

% \begin{table*}[htb]\centering
% \small
% \begin{tabular}{l|rrrrrrrrrrr|c}\toprule
% \textbf{Model} & \textbf{as} & \textbf{gu} & \textbf{kn} &\textbf{ml} & \textbf{mr}& \textbf{or} & \textbf{pa} & \textbf{ta} & \textbf{te} & \textbf{bn} & \textbf{hi} & \textbf{Model-Avg}
% \\\midrule
& \textbf{XLM-RoBERTa}  & \textcolor{BrickRed}{\textbf{66}} & \textcolor{BrickRed}{\textbf{72}} & 70 & \textcolor{BrickRed}{\textbf{68}} & \textcolor{BrickRed}{\textbf{66}} & 65 & \textcolor{BrickRed}{\textbf{72}} & 69 & \textcolor{BrickRed}{\textbf{72}} & 71 &\textcolor{blue}{\textbf{75}}&\textbf{70} \\
& \textbf{IndicBERT} & 63 & 66 & 68 & 61 & 65 & 65 & 66 & 63 & 63 &\textcolor{blue}{\textbf{72}} &\textcolor{blue}{\textbf{72}}& 66 \\
\textbf{English Eval} & \textbf{mBERT-cased} & 62 & 64 & 67 & 65 & 61 & 60 & 66 & \textcolor{BrickRed}{\textbf{67}} & 66 &\textcolor{blue}{\textbf{75}} & 72 & 66 \\
% \S \ref{sec:english_language_model} {RQ2}
& \textbf{MuRIL} & 65 & 33 & \textcolor{BrickRed}{\textbf{71}} & 67 & 67 & \textcolor{BrickRed}{\textbf{67}} & 71 & 31 & 71 & 72 & \textcolor{ForestGreen}{\textbf{77}} & 63 \\
% & \textbf{mBERT-uncased} & 61 & 65 & 61 & 65 & 56 & 66 & 69 & 70 & 67 &\textcolor{ForestGreen}{\textbf{76}}& 74 & 66 \\
\hdashline
& \textbf{LanguageAvg} & 64 & 60 & 68 & 65 & 63 & 64 & 69 & 60 & 68 & 73 &\textbf{74}& 66 \\
\midrule
% \end{tabular}
% \caption{\textbf{English Eval:} model performance (refer \S \ref{sec:english_language_model} {RQ2}). \textbf{Model-Avg} and & \textbf{LanguageAvg} means the same as mentioned in \textbf{table: \ref{tab: translate-Train}}.}\label{tab: translate-test}
% \end{table*}

% \begin{table*}[htbp]\centering
% \small
% \begin{tabular}{l|rrrrrrrrrrr|c}\toprule
% \textbf{Model} & \textbf{as} & \textbf{gu} & \textbf{kn} &\textbf{ml} & \textbf{mr}& \textbf{or} & \textbf{pa} & \textbf{ta} & \textbf{te} & \textbf{bn} & \textbf{hi} & \textbf{Model Avg} \\\midrule

& \textbf{XLM-RoBERTa}  & \textcolor{BrickRed}{\textbf{73}} & 75 & \textcolor{BrickRed}{\textbf{77}} & 75 & \textcolor{BrickRed}{\textbf{74}} & 73 & 75 & 75 & 73 & \textcolor{BrickRed}{\textbf{75}} & \textcolor{ForestGreen}{\textbf{79}} & 76 \\
& \textbf{IndicBERT} & 67 & 72 & 65 & 62 & 59 & 59 &\textcolor{blue}{\textbf{74}} & 63 & 66 & 69 &\textcolor{blue}{\textbf{74}}&70 \\
\textbf{English+\emph{Indic} Train} & \textbf{mBERT-cased} & 67 & 70 & 69 & 70 & 70 & 39 & 71 &\textcolor{blue}{\textbf{73}} & 70 & 70 &71 & 69 \\
% \S \ref{sec:english_language_augmentation}{RQ3} 
& \textbf{MuRIL} & 76 & \textcolor{BrickRed}{\textbf{77}} & 77 & \textcolor{ForestGreen}{\textbf{79}} & 74 & \textcolor{BrickRed}{\textbf{76}} &\textcolor{ForestGreen}{\textbf{77}} &\textcolor{ForestGreen}{\textbf{77}}& \textcolor{BrickRed}{\textbf{74}} & \textcolor{BrickRed}{\textbf{75}} &\textcolor{blue}{\textbf{77}}& \textbf{77} \\
% & \textbf{mBERT-uncased} & 64 & 69 & 63 & 73 & 67 & 35 & 68 & 69 & 68 & 72 & \textcolor{blue}{\textbf{74}} & 69 \\
\hdashline
& \textbf{LanguageAvg} & 69 & 73 & 70 & 72 & 68 & 56 & 73 & 72 & 70 & 72 &\textbf{75} & \textbf{72} \\
\midrule

% \caption{\textbf{English + \emph{Indic} Train:} model performance (refer \S \ref{sec:english_language_model} {RQ3}). \textbf{Model-Avg} and & \textbf{LanguageAvg} means the same as mentioned in \textbf{table: \ref{tab: translate-Train}}.}\label{tab: crosslingual transfer plus translate-Train}


% \begin{table*}[htbp]\centering
% \small
% \begin{tabular}{l|rrrrrrrrrrr|c}\toprule
% \textbf{Model} & \textbf{as} & \textbf{gu} & \textbf{kn} &\textbf{ml} & \textbf{mr}& \textbf{or} & \textbf{pa} & \textbf{ta} & \textbf{te} & \textbf{bn} & \textbf{hi} & \textbf{Model-Avg} \\

% \midrule
& \textbf{XLM-RoBERTa}  &\textcolor{BrickRed}{\textbf{73}} &\textcolor{ForestGreen}{\textbf{77}} &\textcolor{BrickRed}{\textbf{74}} &\textcolor{BrickRed}{\textbf{76}} &72 &73 &\textcolor{blue}{\textbf{77}} &\textcolor{blue}{\textbf{77}}& \textcolor{BrickRed}{\textbf{76}} &\textcolor{blue}{\textbf{77}}&\textcolor{blue}{\textbf{77}} &75 \\
& \textbf{IndicBERT} & 63 & 74 & 59 & 51 & 69 & 66 &\textcolor{blue}{\textbf{75}} & 60 & 67 & 70 & 74 & 66 \\
\textbf{Train All} & \textbf{mBERT-cased} & 63 & 69 & 69 & 71 & 70 & 33 & 71 & 69 & 70 &\textcolor{blue}{\textbf{74}} & 72 & 66 \\
% \S \ref{sec:unified_model} {RQ4}
& \textbf{MuRIL} & \textcolor{BrickRed}{\textbf{73}} & 76 & \textcolor{BrickRed}{\textbf{74}} & \textcolor{BrickRed}{\textbf{76}} & \textcolor{BrickRed}{\textbf{74}} & \textcolor{BrickRed}{\textbf{78}} &\textcolor{ForestGreen}{\textbf{81}} & \textcolor{BrickRed}{\textbf{78}} & \textcolor{BrickRed}{\textbf{76}} & \textcolor{BrickRed}{\textbf{80}} & \textcolor{BrickRed}{\textbf{78}} &\textbf{77} \\
% & \textbf{mBERT-uncased} & 67 & 70 & 69 & 67 & 67 & 40 & 71 & 73 & 67 &\textcolor{blue}{\textbf{75}} & 72 & 67 \\
\hdashline
& \textbf{LanguageAvg} & 68 & 73 & 69 & 68 & 71 & 58 & 75 & 71 & 71 &\textbf{75} & 74 & 70 \\
\bottomrule
\end{tabular}
% \end{tabular}
% \caption{\textbf{Train all:} model performance (refer \S \ref{sec:unified_model} {RQ3}). \textbf{Model-Avg} and \textbf{LanguageAvg} means the same as mentioned in \textbf{table: \ref{tab: translate-Train}}.}\label{tab: translate-Train all}
% \end{table*}
\caption{\footnotesize Here, LanguageAvg represents the language wise average score for all models, while ModelAvg average score represents the average score of the model across all languages. Values in \textcolor{blue}{\textbf{Blue}} represents the model wise average best score across languages, while \textcolor{BrickRed}{\textbf{Red}} represents language-wise average best score across models and \textcolor{ForestGreen}{\textbf{Green}} represents the values where model-wise and language-wise best score coincide. For Indic Cross Lingual Transfer model performance (refer \S \ref{sec:indic_crosslingual}). Every row represent the average evaluation score of all \emph{Indic} language when train on the mentioned column language of \datasetName. For detail results on \emph{Indic} Cross-lingual Transfer refer to Appendix \S\ref{sec:indic_crosslingual_appendix}.
% \da{maybe we can keep english + indic and train all only in main paper and put other technique table in appendix}
}
\label{tab:RQ_1234}
\vspace{-1.0em}
\end{table*}

==> tables_partb.tex <==
\begin{table*}[!htbp]\centering
\small
\begin{tabular}{llrrrrrrrrrrrc}\toprule
\bf{Strategy} & \textbf{Model} & \textbf{as} & \textbf{gu} & \textbf{kn} &\textbf{ml} & \textbf{mr}& \textbf{or} & \textbf{pa} & \textbf{ta} & \textbf{te} & \textbf{bn} & \textbf{hi} & \textbf{ModelAvg} \\\midrule
& \textbf{XLM-RoBERTa}  & 66 & 70 & 33 & 34 & 70 & 35 & 68 & 70 & 70 & 71 & \textcolor{blue}{\textbf{72}} & 60 \\
& \textbf{IndicBERT} & 59 & \textcolor{blue}{\textbf{60}} & 59 & 54 & \textcolor{blue}{\textbf{60}} & \textcolor{ForestGreen}{\textbf{60}} & \textcolor{blue}{\textbf{60}} & 56 & 59 & 58 & \textcolor{blue}{\textbf{60}} & 59 \\
\textbf{\emph{Indic} Train} & \textbf{mBERT cased} & 57 & 59 & \textcolor{blue}{\textbf{60}} & 59 & 58 & 33 & 59 &\textcolor{blue}{\textbf{60}} & 59 & \textcolor{blue}{\textbf{60}} & \textcolor{blue}{\textbf{60}} & 57 \\
& \textbf{mBERT uncased} & 59 & 59 & 60 & 59 & 58 & 33 & 59 & 60 & 60 & 59 & \textcolor{blue}{\textbf{61}} & 57 \\
& \textbf{MuRIL} & \textcolor{BrickRed}{\textbf{75}} & \textcolor{BrickRed}{\textbf{73}} & \textcolor{BrickRed}{\textbf{75}} &\textcolor{ForestGreen}{\textbf{76}}& \textcolor{BrickRed}{\textbf{71}} & 33 & \textcolor{BrickRed}{\textbf{75}} & \textcolor{ForestGreen}{\textbf{76}} & \textcolor{BrickRed}{\textbf{73}} & \textcolor{BrickRed}{\textbf{75}} & \textcolor{BrickRed}{\textbf{73}} & \textbf{70} \\
% & \textbf{mBERT cased} & 57 & 59 & \textcolor{blue}{\textbf{60}} & 59 & 58 & 33 & 59 &\textcolor{blue}{\textbf{60}} & 59 & \textcolor{blue}{\textbf{60}} & \textcolor{blue}{\textbf{60}} & 57 \\
\hdashline
& \textbf{LanguageAvg} & 63 & 64 & 57 & 56 & 63 & 39 & 64 & 64 & 64 &\textbf{65} &\textbf{65} & 60 \\
\bottomrule
\end{tabular}
\caption{Summary of {\emph{Indic} Cross-Lingual Transfer} model performance (refer \S \ref{sec:indic_crosslingual}). Every row represent the average evaluation score of all \emph{Indic} language when train on the mentioned column language of \datasetName. For detail results on \emph{Indic} Cross-lingual Transfer refer to Appendix \S\ref{sec:indic_crosslingual_appendix}. Here, ModelAvg, LanguageAvg, and Color Code mean same as in table \ref{tab:RQ_1234}.}\label{tab:indic_crosslingual_summary}
\vspace{-0.5em}
\end{table*}
